Embodied Concept Learner: Self-supervised Learning of Concepts and Mapping through Instruction Following

Humans, even at a very early age, can learn visual concepts and understand geometry and layout through active interaction with the environment, and generalize their compositions to complete tasks described by natural languages in novel scenes. To mimic such capability, we propose Embodied Concept Learner (ECL) in an interactive 3D environment. Specifically, a robot agent can ground visual concepts, build semantic maps and plan actions to complete tasks by learning purely from human demonstrations and language instructions, without access to ground-truth semantic and depth supervisions from simulations. ECL consists of: (i) an instruction parser that translates the natural languages into executable programs; (ii) an embodied concept learner that grounds visual concepts based on language descriptions; (iii) a map constructor that estimates depth and constructs semantic maps by leveraging the learned concepts; and (iv) a program executor with deterministic policies to execute each program. ECL has several appealing benefits thanks to its modularized design. Firstly, it enables the robotic agent to learn semantics and depth unsupervisedly acting like babies, e.g., ground concepts through active interaction and perceive depth by disparities when moving forward. Secondly, ECL is fully transparent and step-by-step interpretable in long-term planning. Thirdly, ECL could be beneficial for the embodied instruction following (EIF), outperforming previous works on the ALFRED benchmark when the semantic label is not provided. Also, the learned concept can be reused for other downstream tasks, such as reasoning of object states. Project page: http://ecl.csail.mit.edu/

==> figures/ground_vis_bak.tex <==
% \begin{figure}[t]
% \centering
% \footnotesize
% \vspace{1mm}
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_16_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_59_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_46_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_33_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_19_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_18_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/fail_vis/Sem_6_origin.png}~\\
% \vspace{1mm}
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_16_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_59_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_46_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_33_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_19_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_18_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/fail_vis/Sem_6_gt.png}~\\
% \vspace{1mm}
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_16.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_59.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_46.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_33.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_19.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_18.png}~
% \includegraphics[height=.13\columnwidth]{figures/fail_vis/Sem_6.png}~\\
% \vspace{-6pt}
% \caption{Visualization of our concept learning results.
%  From top to bottom: the original image, the learned instance segmentation map with groundtruth as supervisions, and our unsupervised grounded instance segmentation map.
% }
% \vspace{-12pt}
% \label{fig:concept_vis}
% \end{figure}

\begin{figure}[t]
\begin{minipage}[t]{0.32\linewidth}
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm, clip]{figures/ground_acc/concept_small_h.pdf}
    \vspace{-18pt}
    \caption{
    Object grounding accuracy with our concept learning on small objects. 
    % Per-class concept learning accuracy. 
    % (ordered). 
    Results for challenging small objects are shown here. Please refer to the appendix for complete analysis. 
    % More results are included in the Appendix. 
    % and receptacle objects are shown in Appendix. 
    % We show 23 small objects 
    % % (could be picked up) 
    % and the overall accuracy here, more results and the receptacle objects are shown in Appendix.
    }
   \label{fig:concept_small}
    % \vspace{-20pt}
    % \vspace{-9ex}
\end{figure}
\end{minipage}
\hfill
\begin{minipage}[t]{0.3\linewidth} % 37
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/qa/qa_exp.pdf}
    \vspace{-17pt}
    \caption{Examples of concept reasoning and question answering.}
    \label{fig:qa}
\end{figure}
\end{minipage}
\hfill
\begin{minipage}[t]{0.34\linewidth} % 61
\begin{figure}[H]
% \begin{wrapfigure}{R}{0.54\textwidth}
\centering
\footnotesize
% \vspace{-42pt}
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_16_origin.png}~
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_59_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_46_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_33_origin.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_19_origin.png}~
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_18_origin.png}~
\includegraphics[height=.235\columnwidth]{figures/fail_vis/Sem_6_origin.png}~\\
\vspace{1mm}
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_16_gt.png}~
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_59_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_46_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_33_gt.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_19_gt.png}~
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_18_gt.png}~
\includegraphics[height=.235\columnwidth]{figures/fail_vis/Sem_6_gt.png}~\\
\vspace{1mm}
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_16.png}~
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_59.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_46.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_33.png}~
% \includegraphics[height=.13\columnwidth]{figures/ground_vis/Sem_19.png}~
\includegraphics[height=.235\columnwidth]{figures/ground_vis/Sem_18.png}~
\includegraphics[height=.235\columnwidth]{figures/fail_vis/Sem_6.png}~\\
\vspace{-6pt}
\caption{Visualization of our concept learning results.
 From top to bottom: the original image, the learned instance segmentation map with groundtruth as supervisions, and our unsupervised grounded instance segmentation map.
}
\vspace{-12pt}
\label{fig:concept_vis}
\end{figure}
% \end{wrapfigure}
\end{minipage}
\vspace{-10pt}
\end{figure}

==> tables/ablation.tex <==
\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{9pt}
\renewcommand\arraystretch{1.15}
\caption{Ablation on semantic grounding 
}
\resizebox{1\linewidth}{!}{
    \begin{tabular}{l|ccccc}
    % \toprule
    \shline
    \multirow{1}{*}{Method} & Grounding Acc. & PLWGC & GC & PLWSR & SR \\
    \shline
    Learned Encoding & 49.1 & 10.57 & 25.40 & 6.87 & 15.89 \\
    Word Embedding & \textbf{57.6} & \textbf{11.11} & \textbf{27.30} & \textbf{7.30} & \textbf{17.24} \\
    \shline
    \end{tabular}
    }
    \label{tab:ablation1}
\end{table}



\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand\arraystretch{1.15}
\caption{Ablation on mapping Test Unseen Only.}
\resizebox{1\linewidth}{!}{
    \begin{tabular}{l|cccc}
    % \toprule
    \shline
    % Method  & sup. mono. depth  & unsup. mono. depth & PLWGC & GC & PLWSR & SR \\
    Method  &  PLWGC & GC & PLWSR & SR \\
    \shline
    % Mono. depth  & 11.11 & 27.30 & 7.30 & 17.24 \\
    % \hline
    Maximum Fusion~\cite{min2021film} + Unsup. Mono. Depth & 6.03 & 16.57  &2.82 & 7.39 \\
    Bayesian Filtering (Ours) + Unsup. Mono. Depth   &10.87 &19.83 &4.17 & 9.03\\
    % Moving Avg~\cite{}+unsup mono depth  & \\
    \shline
    \end{tabular}
    }
    \label{tab:ablation}
\end{table}

==> tables/count_task.tex <==
\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.15}
\caption{Counting accuracy. Transfer to other task. learning concept, Reasoning (example, same room, which room)
}
\resizebox{0.5\linewidth}{!}{
    \begin{tabular}{lccc}
    % \toprule 32
    \shline
    \multirow{1}{*}{Model}  & Grounding & Exist & Count \\
    \shline
    Random Guess & -- & 50.0\% & 25.0\% \\
    C3D~\cite{tran2015learning}  & -- &  & 34.4\% \\
    \alias (Ours) & 57.6\%  &  &  56.3\%\\
    \shline
    \end{tabular}
    }
    \label{tab:count}
\end{table}


==> tables/error_modes.tex <==
\begin{table}[t]
\centering
\fontsize{8}{8}\selectfont
\setlength\tabcolsep{4pt} 
\captionof{table}{\textbf{Error Modes}. The percentage of failure cases belonging to different failure modes for ECL on the validation set.}
\vspace{-0.3em}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Error mode}
   &\multicolumn{1}{c}{\textbf{Seen \%}} && \multicolumn{1}{c}{\textbf{Unseen \%}} \\
\midrule
% \;Target not found              &9.28   &&12.88  \\    %
\;Target not found              &36.38   &&28.53  \\    %
\;Interaction failures          &6.59   &&10.39\\    %
\;Collisions                    &4.34   &&4.43\\    %
\;Blocking/Object not accessible &31.29 &&39.75  \\    %
% \;Exceed step limit             &27.10  &&15.65\\
% \;Language processing error  \\    %
\;Others                        &21.41  &&16.90\\    %
               
\bottomrule
\end{tabular}
\label{tab:error_modes}
\end{table}

% \begin{table}[t]
% \centering
% \fontsize{8}{8}\selectfont
% \setlength\tabcolsep{4pt} 
% \captionof{table}{\textbf{Error Modes}. Table showing percentage of errors due to each failure mode for FILM on the Val set. \my{xuyan}}
% \vspace{-0.3em}
% \begin{tabular}{@{}lccc@{}}
% \toprule
% \textbf{Error mode}
%   &\multicolumn{1}{c}{\textbf{Seen \%}} && \multicolumn{1}{c}{\textbf{Unseen \%}} \\
% \midrule
% \;Goal object not found  \\    %
% \;Interaction failures \\    %
% \;Collisions  \\    %
% \;Object in closed receptacle   \\    %
% \;Language processing error  \\    %
% \;Others \\    %
               
% \bottomrule
% \end{tabular}
% \label{tab:error_modes}
% \end{table}
